American cities are defined by isolated rings and pockets characterized by limited socio-economic mixing

Cities generate gains from interaction, but citizens often experience segregation as they move around the urban environment. Using GPS location data, we identify four distinct patterns of experienced segregation across US cities. Most common are affluent or poor neighborhoods where visitors lack diversity and residents have limited exposure to diversity elsewhere. Less frequent are majority-minority areas where residents must travel for diverse encounters, and wealthy urban zones with diverse visitors but where locals sort into homogeneous amenities. By clustering areas with similar mobility signatures, we uncover rings around cities and internal pockets where intergroup interaction is limited. Using a decision tree, we show that demography and location interact to create these zones. Our findings, persistent across time and prevalent across US cities, highlight the importance of considering both who is mixing and where in urban environments. Understanding the mesoscopic patterns that define experienced segregation in America illuminates neighborhood advantage and disadvantage, enabling interventions to foster economic opportunity and urban dynamism.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
